Cross-domain Neural Pitch and Periodicity Estimation

Pitch is a foundational aspect of our perception of audio signals. Pitch contours are commonly used to analyze speech and music signals and as input features for many audio tasks, including music transcription, singing voice synthesis, and prosody editing. In this paper, we describe a set of techniques for improving the accuracy of widely-used neural pitch and periodicity estimators to achieve state-of-the-art performance on both speech and music. We also introduce a novel entropy-based method for extracting periodicity and per-frame voiced-unvoiced classifications from statistical inference-based pitch estimators (e.g., neural networks), and show how to train a neural pitch estimator to simultaneously handle both speech and music data (i.e., cross-domain estimation) without performance degradation. Our estimator implementations run 11.2x faster than real-time on a Intel i9-9820X 10-core 3.30 GHz CPU$\unicode{x2014}$approaching the speed of state-of-the-art DSP-based pitch estimators$\unicode{x2014}$or 408x faster than real-time on a NVIDIA GeForce RTX 3090 GPU. We release all of our code and models as Pitch-Estimating Neural Networks (penn), an open-source, pip-installable Python module for training, evaluating, and performing inference with pitch- and periodicity-estimating neural networks. The code for penn is available at https://github.com/interactiveaudiolab/penn.

==> reviewer-comments.tex <==
Reviewer: 2

Recommendation: RQ - Review Again After Major Changes

Comments:
Compared to the previous submission, the manuscript has significantly improved. However, there is still a long way to go. Although my comments may sound harsh (apologies for this), I have to admit that it is only in this version of the manuscript that I am able to identify the major problem with it.

The aim of the manuscript is to proposes a framework that can efficiently estimate pitch and periodicity for both speech and music. So there are two critical questions should be answered: 1) what method enables the estimation of pitch and periodicity across speech and music; 2) what method enables the estimation of pitch and periodicity in an efficient way. The author should describe and justify the method proposed for achieving the proposed objectives. 

More specific suggestions are as the following:

1. Regarding to the “out-of-domain”, though this version of manuscript has successfully described what domain means but the term “multi-task” is still a more accurate term given the context of pitch estimation of speech and music. The author is also encouraged to investigate why methods for speech usually do not work well for music, which could be taken as the motivation of the manuscript and the proposed method. 

2. The introductory section is not a section to provide background information. The author should address the key technical problem proposed and the respective solution proposed. The author should also address the experiment proposed to demonstrate the proposed scientific hypothesis and the expected result that can be used as the evidence of the demonstration process. The current manuscript only uses three paragraphs (as a list with bullet points) to do so, which falls short of expectation.

3. Section III current severs as a distraction of readers’ attention. The small tricks applied should not occupy more than a column unless the proposed tricks has supported the main tasks i.e., the ability of processing both speech and music, and, the improvement on efficiency of processing. 

4. On the contrast, section IV should be extended as to my best knowledge (or to my best guess), the methods proposed in this section lead to the ability of processing both speech and music and the efficiency of processing. The author should justify why the proposed method would lead to the proposed objectives and use auxiliary experiments (such as the experiment presented by Figure 3) to demonstrate the hypothesis is true.

5. Regarding to Figure 3, the only experiment presented as an evidence / a support to a scientific hypothesis, the author should give more detailed description on how the result presented by figures is obtained. For example, there are no explanations on the number presented at the bottom of each diagram. The author should also clearly justify why the experiment is proposed (i.e., the objective of the experiment) and demonstrates how the result can be interpreted as evidence supporting the hypothesis proposed.

To respond to the rebuttal from the author in the last round, a scientific hypothesis is a proposed explanation for a result of experiment. It is a tentative explanation for an observation or scientific problem that can be tested through experimentation. Usually the scientific hypothesis should be in a form of “Method A helps Task B because of Reason C”. The technical tricks improving the general performance are not considered as scientific hypothesis regardless of how many tricks are there and how significant the improvements are.

Another minor comments about the use of pronoun: the reduced use of pronoun such as “we” and “our” does improve the readability of the manuscripts. However, there are still minor parts that two sentences starts with “we” or “our”. The author may want to pay attention to this particular point when a significant part of the manuscript is re-written.

In general, this revised manuscript is on the right track of being accepted. There are a few supplementary experiments are suggested to demonstrate the effects of the proposed methods together with a few major re-organisation of the manuscript. I encourage the author to revise the manuscript and then re-submit the manuscript again. By which time, I hope the manuscript could be awarded an “AQ” or an “A”.

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Not Novel

Explain: The paper proposes a framework of pitch and periodicity estimation. The author does not provide a description on which section of the framework is novel or what method is proposed to make an improvement on the performance of pitch and periodicity estimation. As a result, it is impossible to estimate the novelty of the paper.

3. Is the contribution significant?: Incremental

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Important Information is missing or superficially treated

5. Rate the Bibliography: Satisfactory

If you are suggesting additional references they must be entered in the text box provided.  All suggestions must include full bibliographic information plus a DOI.
: N/A

1. How would you rate the overall organization of the paper?: Could be improved

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

4. Are symbols, terms, and concepts adequately defined?: Yes

5. How do you rate the English usage?: Satisfactory


Reviewer: 1

Recommendation: AQ - Publish With Minor, Required Changes

Comments:
The paper contributes a systematic comparison, analysis, and optimization of current state-of-the-art neural pitch estimation methods. Further novelty is provided by the proposed entropy-based voicing detector. In addition, the provided open-source implementations of the studied methods are both valuable for the research community, and also likely  attract citations to the paper. 

Current revised version of the manuscript addresses review comments sufficiently and the paper is in good polished state. 

Few minor typographical suggestions follow

1) In Eq. 7
Should the greater-than symbol be less-than instead? Now it looks like you get a point for accuracy if the pitch difference is larger than the threshold.

2) In References,
- Capitalise Viterbi as a proper noun in [24]
- Check that capitalisation is as intended in [35], [36], [42]
- [51] is a GitHub repository, but missing an URL

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: The paper contributes a systematic comparison, analysis, and optimization of current state-of-the-art neural pitch estimation methods. Further novelty is provided by the proposed entropy-based voicing detector. In addition, the provided open-source implementations of the studied methods are both valuable for the research community, and also likely attract citations to the paper.

3. Is the contribution significant?: Moderately Significant

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Yes

5. Rate the Bibliography: Satisfactory

If you are suggesting additional references they must be entered in the text box provided.  All suggestions must include full bibliographic information plus a DOI.
: References are adequate.

1. How would you rate the overall organization of the paper?: Satisfactory

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

4. Are symbols, terms, and concepts adequately defined?: Yes

5. How do you rate the English usage?: Satisfactory


Reviewer: 3

Recommendation: A - Publish Unaltered

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: 

1. Is the paper technically sound?: 

2. How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: See report

3. Is the contribution significant?: 

4. Is the coverage of the topic sufficiently comprehensive and balanced?: 

5. Rate the Bibliography: 

If you are suggesting additional references they must be entered in the text box provided.  All suggestions must include full bibliographic information plus a DOI.
: Good

1. How would you rate the overall organization of the paper?: 

2. Are the title and abstract satisfactory?: 

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: 

4. Are symbols, terms, and concepts adequately defined?: 

5. How do you rate the English usage?:
